The Hidden Adversarial Vulnerabilities of Medical Federated Learning

In this paper, we delve into the susceptibility of federated medical image analysis systems to adversarial attacks. Our analysis uncovers a novel exploitation avenue: using gradient information from prior global model updates, adversaries can enhance the efficiency and transferability of their attacks. Specifically, we demonstrate that single-step attacks (e.g. FGSM), when aptly initialized, can outperform the efficiency of their iterative counterparts but with reduced computational demand. Our findings underscore the need to revisit our understanding of AI security in federated healthcare settings.

==> 1.5_Preliminaries.tex <==
\section{Preliminaries and related works}
\label{sec:prelimianries}
\subsection{Federated Learning}


Federated learning enables multiple data owners with private datasets to jointly train a global model based on local models. The  optimization problem could be formulated as
${w} = \sum\limits_{i=1}^{N}{p_{i}{w}_{i}}$ , ${w}_{i}=\arg\min\limits_{{w}_{i}}{\left(\mathcal{L}(\mathcal{D}_{i};{w})\right)}$ where $N$ is the number of data owners, $\mathcal{L}(\mathcal{D}_{i};{w})$ is a loss function indicating global model parameters  ${w}$ of local datasets.  
 The learning procedure is an iterative process containing local and global steps. Each data owner trains a model received from a global server on its local dataset in local iterations. The global server updates the global model by aggregating the updated local models. Then it sends it back to clients for the next round. 
 
 The global server selects a subset of clients at each global round and sends the most recent global model to them. Then each client performs local training over its dataset for a selected number of epochs. The updated local models are calculated on selected batches. Local optimization can be formulated as ${w}_i \leftarrow {w}-\eta\cdot \nabla \mathcal{L}({w};\mathcal{D}_{i})$, where 
%  $\beta$ is a batch randomly sampled from the local dataset and
 $\eta$ is the learning rate. Several local iterations might be required to go over all the local data. Local training procedures can be done for several local epochs.
%
(3) The global model can be updated based on the local models ${w}_i$ and is shared for aggregation: 
${w} = \sum\limits_{i=1}^{N}{p_{i}{w}_{i}}$, to update the global model for the next federated round.


Differential privacy (DP) requires federated learning parties to ensure an attacker can not distinguish data records. For multi-party systems $\mathcal M: \mathcal{X}\rightarrow \mathcal{R}$ mapping from domain $\mathcal{X}$ to target domain $\mathcal{R}$, differential privacy  $(\epsilon, \delta)$-DP defines a measure to evaluate  performance of privacy preserving mechanisms.
For two adjacent datasets $\mathcal D_i, \mathcal D_i'$. DP introduces a bounding parameter $\epsilon > 0$ , representing the ratio of probabilities of two datasets bounded by performing the privacy preserving mechanism  $\delta$. It can be summarized by the following definition \cite{dwork2014algorithmic}:
 
\begin{definition}
Mapping $\mathcal M: \mathcal{X}\rightarrow \mathcal{R}$ is $(\epsilon, \delta)$-DP,
if for all measurable subsets of target domain $\mathcal S\subseteq \mathcal{R}$ and for any two adjacent datasets $\mathcal D_i, \mathcal D_i'\in \mathcal{X}$, 
\begin{equation}\label{equ:Differential privacy}
\emph{Pr}[\mathcal M(\mathcal D_i)\in \mathcal S]\leq e^{\epsilon}\emph{Pr}[\mathcal M(\mathcal D_i')\in \mathcal S]+\delta.
\end{equation}
\end{definition}
% As a guaranteed way to obtain $(\epsilon, \delta)$-DP, gaussian mechanism proposed in \cite{dwork2014algorithmic} can be used. 
In FL setting,  $(\epsilon, \delta)$-DP can be achieved by adding noise to the updated models.
% To ensure privacy for both global server and clients,
Global differential privacy is a privacy mechanism that imposes a double-sided $(\epsilon, \delta)$-DP requirement for both uplink and downlink channels\cite{wei2020federated}.
From the uplink perspective, all clients $1\leq i\leq N$, clip their updates  $\Vert{w}_{i}\Vert \leq C$, where ${w}_{i}$ denotes the updated weights from the $i$-th client before perturbation and $C$ is the clipping threshold. To satisfy a $(\epsilon, \delta)$-DP requirement for the downlink channels, additional noise ${n}_{\text i}$ is   added by the server, so each client $i$ receives a $\tilde{w_i}$ perturbed model\cite{wei2020federated}.

 
%  ing ${w}_{i}$. 
%  and ${w}$ are the aggregated parameters at the server to be broadcast to the clients.

%===========================================================================

% \subsection{Adversarial attacks}


\subsection{Adversarial attacks }

Introduced by \cite{szegedy2013intriguing}, 
adversarial examples are feature space manipulations with respect to linear decision boundaries,
\cite{goodfellow2014explaining} and are categorized based on the adversary's goal and knowledge.
\\\textbf{Adversary's goal} Adversarial attacks can be categorized based on the adversary's goal. \textit{Untargetted attacks} aim to reduce the model performance,  regardless of the class to which a test sample belongs. \textit{Targeted attacks} force the model to output certain labels.
\\\textbf{Adversary's knowledge} Based on the adversary's knowledge, the attack can be  \textit{white-box},
meaning that the adversary has complete knowledge about other clients' network architecture, gradients, and parameters. In such a setting, it can easily manipulate the model. White-box attacks have been extensively investigated in the literature\cite{xu2020adversarial}. In \textit{black-box} heuristics, the adversary does not have access to the target model. In the black-box setting, however, it can interact with the model. Adversary can feed inputs and receive outputs of the target model and improve the attack by observing the model outputs. Some black box might have limited knowledge about design of the target model\cite{yue2021black,9000972,cheng2019improving}.
% attack can be \textit{black-box},  meaning that the adversary does not know about the model parameters or gradients of the victim network, but can interact with the model and query its output for given samples. adversary, has full knowledge about the victim network, including its layer weights and and parameters. White-box adversaries are the most powerful ones.
% Numerous adversarial attacks have been proposed in the literature in order to fool deep neural networks and produce false predictions. Adversarial attacks work through injecting a guided imperceptible noise that fools the trained deep learning model.
\\Popular attack methods are Projected Gradient Descent (PGD), Fast Gradient Sign Method (FGSM), and Basic Iterative Method (BIM). Each will be discussed in this section.

\textbf{FGSM:} Fast Gradient Sign Method (FGSM) \cite{szegedy2013intriguing} is a fast yet effective method which produces adversary images with one step of calculation. Assuming input $x$ and its corresponding target $t$, FGSM calculates gradient of $x$ with respect to the loss function ${\partial \mathcal{L}}/ \partial {x}$.

\begin{equation}
\label{eqt:fgsm}
    \bm{\hat{x}} = \bm{x} + \epsilon \cdot sgn\big(\nabla_{\bm{x}}{\mathcal{L}}(g(\bm{x};w)\big)
\end{equation}

where epsilon $\epsilon$ is a hyper-parameter which determines adversarial noise level. $g(\bm{x};\bm{w})$ is the output of neural network with respect to the input $x$ and parameter set $w$. $sgn(.)$ is the sign function. The result of sign function goes through a clipping function to impose a maximum bound in change to the perturbation $\epsilon \cdot sgn\big(\nabla_{\bm{x}}{\mathcal{L}}(g(\bm{x};\bm{w})\big)\in [-1,1]$.

\textbf{BIM:}  Basic Iterative Method (BIM) is an extension of the FGSM method, proposed by Kurakin et al.\cite{kurakin2018adversarial}. BIM repeatedly performs the FGSM process, using a small step-size and $\bm{\hat{x}^{1}} = \bm{x}$. BIM is stronger than FGSM and requires smaller perturbations.

\textbf{PGD:} Madry et al.  proposed their own version of the BIM attack. In Projected Gradient Descent (PGD) \cite{madry2017towards}
the attack starts with a uniform random initialization. The update formula for PGD attack can be written as: 
\begin{equation}
\label{eqt:pgd}
    \bm{\hat{x}}^{t+1}=\Pi_{P_\epsilon(\bm{x})} \Big( \bm{\hat{x}}^t + \alpha \cdot sgn\big(\nabla_{\bm{x}}{\mathcal{L}}(g(\bm{\hat{x}}^t;\bm{w}),t)\big)\Big)
\end{equation}
Where $\bm{\hat{x}}^{k}$ is the perturbed data in $k$-th iteration, and $P_\epsilon(\bm{x})$ is the projected gradient descent function, which is done by first finding sign values and then projecting the result to a small neighborhood of the input ${x}$. These possible parameter spaces determine the set of PGD attack samples that an adversary can use. PGD is one of the strongest attacks and is a universal first-order adversarial method. Technically, PGD is similar to BIM but with a small random initialization, aside from formulating the problem as a projected gradient. We report results with PGD. With equal iterations, BIM had the same results, or the difference was negligible.

==> 2_Relatedworks.tex <==
\subsection{Medical imaging domain}
\label{sec:related}
% 

The effect of adversarial attacks on medical image analysis has been studied in several works. Tasks such as chest X-ray, MRI \cite{finlayson2019adversarial,bortsova2021adversarial,asgari2018vulnerability,ma2021understanding} and CT scan
\cite{navarro2021evaluating}
  segmentation and classification are vulnerable to adversarial attacks \cite{ozbulak2019impact}.
\\Several studies were performed to discover important parameters related to attack transferability\peter{What is meant by that? Should be useful for the reader to explain what "attack transferability" means.}\quickthings{Added the definition in the introduction}
\cite{gao2022boosting}. Gradients of different samples in one batch, extent of data augmentation \cite{gao2022boosting}, variation in input gradients \cite{qiu2022framework} have been shown to be important in transferability. Zhang et al. analyzed the impact of transfer learning methods on black-box attack \cite{zhang2020two}. Another work \cite{zheng2020efficient} utilized the transferability of adversarial examples to enhance  robustness, although their method was proposed for a white-box setting. 

% The effectiveness of the above methods is not apparent in the federated setting.




In medical image analysis,  perturbation degree
has been shown previously as a less explored but highly deterministic parameter in attack setting, and might need visual tuning \cite{bortsova2021adversarial}. Optimal values of standard black-box\cite{bortsova2021adversarial}, and white-box \cite{ma2021understanding} are domain-specific. Also iteration steps $\alpha$, can be highly deterministic in centralized setting \cite{tashiro2020diversity} \cite{cai2018curriculum}. 
% \textbf{Adversarial attacks on Federated learning} 
 
% \\Also, some enhancement methods have been proposed. 

 
Methods such to detect the attack
\cite{yin2021exploiting,drenkow2022attack,ma2021understanding }
or defend the models from adversaries\cite{lin2021certified,yuan2019adversarial,papernot2017practical,biggio2018wild,li2022review} were also discussed in the ML domain.
 Adding noise to the exchanged model with clipping model updates is effective in several forms of adversarial attacks \cite{bouacida2021vulnerabilities}. In norm-bound defense, the server enforces an upper-limit norm-bound. Several studies have investigated black-box PGD attacks in a federated environment with norm-bound situation \cite{sun2019can,wang2020attack}. In the clinical setting,
% Some models have proposed differentially private settings.
\cite{shao2019stochastic} DP models are used in clinical EHR data\cite{li2019distributed}  \cite{ma2019privacy} and neuroimaging data \cite{li2020multi} in multi-site setting. 



% and less evaluated in MIA domain.
% \\\hl{Yejuri in kosshere CVPR ro biar ke na sikh besuze na kabab}

% \\\hl{\faClockO bebin stucking ro mituni biari,Using knowledge from previous rounds / stacing:
% age na inaro biar:
% \\\faQuestion Effect of perturbation degree ro kia barresi kardan
% \\\faQuestion Effect of alpha ro kia barresi kardan
% }
% \\\hl{\faClockO Maqalati ke asare noise level be FL tajihan}\\
% \hl{\faClockO Maqalati sanjidan number of clients ro sanjidan}\\
% \hl{\faClockO Other attacks on MI has been done}\\
% \hl{\faClockO Some privacy attacks on FL MI has been done}




==> 4_results.tex <==
\section{Results}


\label{sec:results}




% Original images, adversarial images, and corresponding adversarial noise created with FGSM ( ϵ=0.02) in different black-box settings


\subsection{Efficiency analysis}


\begin{figure*}[h!]
     \centering
     \begin{subfigure}[b]{0.99\textwidth}
         \centering
         \includegraphics[width=0.32\textwidth]{photo/Meningioma_ASR_EPS_steps.eps}
          \includegraphics[width=0.32\textwidth]{photo/Glioma_ASR_EPS_steps.eps}
           \includegraphics[width=0.32\textwidth]{photo/Pathology_ASR_EPS_steps.eps}
         \caption{Average ASR on benign clients }
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.99\textwidth}
          \centering
         \includegraphics[width=0.32\textwidth]{photo/Meningioma_others_EPS_steps.eps}
          \includegraphics[width=0.32\textwidth]{photo/Glioma_others_EPS_steps.eps}
           \includegraphics[width=0.32\textwidth]{photo/Pathology_others_EPS_steps.eps}
         \caption{Average ASR on advesarial client }
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
        \caption{Effect of Error perturbation step $\alpha$ on attack transferability. PGD attack with and without CRN initialization was performed. ASR is calculated on benign and adversary clients.The higher ASR on benign clients shows higher transferability}
        \label{fig:three graphs}
\end{figure*}

The models are trained in a federated environment. Average test results, or clean accuracy shows the average performance of clients on unperturbed test data. 
% This could be a baseline for comparison of attacks.
Here we compare the computational complexity of iterative algorithms. The comparison is based on the time required to train one batch of adversarial examples, with  $\epsilon=0.05$ and $\alpha=0.001$. 
As table \ref{table_time} shows, the higher iteration rounds take more computation and lead to higher AASR. 
% Also, CRN does not require additional computation. Similar to single-step methods, computational load is small but increases on high-resolution images. As an example, the pathology dataset requires more calculation than MRI data. 
However, the overall time is far less than iterative models, and also it could enhance the transferability much better. The effect is consistent among different datasets. 
% However,  This means that Pathology images have better AASR than MRI images in baseline and CRN enabled attacks.
% Also,  

% PGD can sometimes perform poorly, even in higher iterations. Enabling the initialization might  


\begin{table}[h!]
\centering
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1.22}
\caption{ \small Comparison of iterative models and their computational efficiency, on performing computations on one batch of data.  ACC shows average client performance for unperturbed test data. AASR is average ASR on all clients.\peter{Can you add how these attacks effect the global model's performance in terms of accuracy? Same for plots below. Your adversary's stated goal is to reduce accuracy of the global model. That goal should be aligned with the experimental results. }\quickthings{AASR is exactly what you are referring to. For example in this table 63.92 \% AASR means the average success of attacker for  }
}
\begin{tabular}{| *{5}{c|} }
\hline
Dataset  & Attack type & ACC & AASR & time (sec)
\\   \hline  
\multirow{3}{5em}{Meningioma}     &\textbf{PGD-1+CRN10}&\multirow{3}{3em}{84.12\%}&\textbf{63.92\%} & \textbf{0.217}  \\
 &PGD-20&&27.52\% & 3.423 \\
&PGD-40&&32.99\% & 6.794  \\ \hline
\multirow{3}{4em}{Pathology}     &\textbf{PGD-1+CRN10}&\multirow{3}{3em}{77.01\%}&\textbf{90.92\%} & \textbf{0.354} \\
&PGD-20&&60.98\% & 5.464\\
&PGD-40&&82.27\% & 10.843 \\ \hline
\multirow{3}{3em}{Glioma}     &\textbf{PGD-1+CRN10}&\multirow{3}{3em}{61.84\%}&\textbf{70.55}\% & \textbf{0.216}  \\
&PGD-20&&51.83\% &3.420  \\
&PGD-40&&63.77\% & 6.793  \\ \hline


\end{tabular}
\label{table_time} 
\end{table}




\subsection{Effect perturbation degree}

We performed attack scenarios to evaluate the effect of perturbation degree $\epsilon$  on attack success on the model. We compared the baseline attack to CRN- enabled attacks. ASR is calculated on benign and adversary clients and is shown in Fig \ref{fig: epsilon graphs}.

More successful attacks on adversaries led to higher transferability to benign clients. Low values of $\epsilon$ can decrease transferability to a large extent. $\epsilon$ = 0.01 has lower ASR rates on all the clients. Generally, Higher $\epsilon$ values lead to higher ASR in all scenarios. 
In pathology images, Iterative models can reach perfect accuracy on the adversarial client and have very high transferability.

CRN  has a positive effect on transferability in all scenarios. Also, CRN-enabled models are more dependent on $\epsilon$; their extent can vary depending on the dataset, attack method, and value of $\epsilon$.
Tuning $\epsilon$  might be tricky since performance and imperceptibility should be considered together.High $\epsilon$ values mean more distortion in the image. We performed an FGSM attack with varying $\epsilon$ values to evaluate the perturbation effect visually. Fig. \ref{fig:perturbedMRI} shows the results of perturbed images with different perturbation degrees and their comparison with the unperturbed image. Note that perturbation values below  $\epsilon=0.05$ cause limited distortion. Iterative models can reach high ASR very quickly with increasing $\epsilon$. 

\begin{figure*}[h!]
 \centering
 \includegraphics[width=0.8\textwidth]{photo/Adversarial_attacks-5.eps}
 \caption{\small From (a) to (f), normal tumor image, and perturbed images with FGSM attack, with perturbation parameters: $\epsilon$ = 0.01, 0.03, 0.05,  0.10, respectively \peter{Also, it looks like this figure wasn't referenced in the text.} \quickthings{Added to the dicussion part b}}
 \label{fig:perturbedMRI}
\end{figure*}











% \subsection{AATR}
% \begin{table}[h]
% \centering
% \setlength{\tabcolsep}{8pt}
% \renewcommand\arraystretch{1.4}
% \caption{Result of our experiments for PGD attack on Pathology data $\epsilon$ values. The iterative models are trained for 40 rounds with step size of 0.01. \hl{\faQuestion maybe you can change the word for without CRN}}
% % \begin{tabular}{cccccccccccc}
% \begin{tabular}{| *{4}{c|} }\hline
% % Dataset  & Attack type & \multicolumn{2}{c|}{ $\epsilon=0.01$} & \multicolumn{2}{c|}{ $\epsilon=0.03$}           &    \multicolumn{2}{c|}{ $\epsilon=0.05$}    & \multicolumn{2}{c|}{ $\epsilon=0.07$}                                                              \\ \hline
%  Dataset&\multicolumn{3}{c|}{ FGSM}    
% %  &              \multicolumn{3}{c|}{ PGD}                                                                           \\  

%  \cline{2-5}
% &Baseline&CRN5 &CRN10\\\hline

% Meningioma&84.80\%&\textbf{86.31}\%&{84.02\%}
% % \%&83.73\%  &\textbf{84.25}\%  &84.16\%
% \\\hline
% Glioma&82.32\% &87.06\%&\textbf{89.98\%}
% % &74.89\%&\textbf{83.64}\% &82.32\%
% \\\hline

% Pathology&\textbf{90.67\%}&{84.81\%}\%&{85.98\%}
% % \%&79.86\% &86.79\%&\textbf{86.93\%}
% \\\hline



% \end{tabular}
% \label{table_core} 
% \end{table}










\subsection{Effect perturbation step}


Another critical parameter is the step of change in iterative methods ({$\alpha$}), which is shown to be highly deterministic in specific settings but is not yet investigated in medical image analysis domain. To evaluate how $\alpha$ can affect transferability, we examined the clients with $\epsilon =0.03$ in various steps. Generally, there is an optimal middle range the same as $\epsilon$. A step size of 0.007 led to the highest transferability in MRI images. Larger steps led to a sharp decrease in transferability. For pathology images, about 0.007 led to the best ASR on the adversary, and higher values decreased both ASR on adversary and transferability. However, smaller steps also had high ASR values. 







\subsection{Error tranferability}


We also evaluated another performance metric, the average error transfer rate (AETR). Although  PGD method surpasses the FGSM in terms of attack success rate, their AETR values are comparable. The PGD method is trained for 40 iterations, and the models are evaluated both with and without the Cross-round Noise (CRN).

The observation that both FGSM and PGD exhibit high AETR implies that, despite FGSM potentially generating less optimal adversarial examples in general, the instances that successfully deceive the adversary are also highly transferable to benign clients. The inclusion of CRN tends to increase the AETR, further highlighting the effectiveness of the cross round initialization.

 

\

\begin{table*}[h!]
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand\arraystretch{1.4}
\caption{Result of Average Error Transfer Rate (AETR) for FGSM and PGD methods, with and without CRN initalization. Each number is the average result for three experiments.} \peter{What is the baseline attack?}\quickthings{ Vanilla FGSM without the proposed initalization, I have changed the wordings in the table} 
% \begin{tabular}{cccccccccccc}
\begin{tabular}{| *{7}{c|} }\hline
% Dataset  & Attack type & \multicolumn{2}{c|}{ $\epsilon=0.01$} & \multicolumn{2}{c|}{ $\epsilon=0.03$}           &    \multicolumn{2}{c|}{ $\epsilon=0.05$}    & \multicolumn{2}{c|}{ $\epsilon=0.07$}                                                              \\ \hline
 Dataset&\multicolumn{3}{c|}{ FGSM}     &              \multicolumn{3}{c|}{ PGD}                                                                           \\  

 \cline{2-7}
&Vanilla&CRN5 &CRN10&Vanilla&CRN5&CRN10\\\hline

Meningioma&84.80\%&\textbf{86.31}\%&{84.02}\%&83.73\%  &\textbf{84.25}\%  &84.16\%\\\hline
Glioma&82.32\% &87.06&\textbf{89.98\%}&74.89\%&\textbf{83.64\%}\% &82.32\%\\\hline

Pathology&\textbf{90.67\%}&{84.81}\%&{85.98}\%&79.86\% &86.79\%&\textbf{86.93\%}\\\hline



\end{tabular}
\label{table_core} 
\end{table*}




==> 5_discussion.tex <==


\section{Discussion}
\label{sec:discussion}
Our results confirm  prior research about vulnerability of FL networks
\cite{goldblum2020dataset,miotto2016deep,costa2021covert,bouacida2021vulnerabilities,darzidehkalani2022federatedeco} and medical image analysis systems\cite{finlayson2019adversarial,gupta2022vulnerability,bortsova2021adversarial}  to adversarial attacks.

% Our results suggest that even in a DP-enabled setting, adversarial samples generated on one client can be highly transferable.

We also found that differential privacy might have partial effect on attacker's success. In fact, DP caused the lower ASR in benign than the adversary clients.
% But it can not be considered as an effective counter-measure.
Although some research supports DP, our findings suggest that it is an option but not very reliable \cite{bouacida2021vulnerabilities,darzidehkalani2022federated2}.Additionally, it is important to consider the accuracy compromise that arises from the noise introduced by DP. This trade-off between privacy protection and model performance should be carefully evaluated, as excessive noise could negatively impact the model's overall accuracy and effectiveness in real-world applications.
\\In our experiments the attacker did not tamper with the training procedure. This is unlike backdoor or poisoning attacks \cite{lyu2020privacy}\cite{lyu2020threats}, where the attacker performs malicious activities during training, and opens the way for detection methods.
Also, CRN initialization led to faster attacks with higher transferability. This section discusses our findings, how they could be important in the medical imaging domain, and what to consider when setting up federated medical image analysis infrastructure.



\subsection{Transferability}
% The practice could be that not always adding noise is better, especially in medical images where compromising accuracy affects patients. Other methods have their problems as stated before, \cite{yin2022adc,yuan2019adversarial,uesato2018adversarial} mainly compromising performance or working in certain conditions. 
% Further research might consider defense models of FL networks. 
Our experiments aimed to asses some factors in transferability. However, in addition to the investigated factors, we found three other parameters that might highly predict transferability.



\textbf{Benign/Adversary correlation:} Our results show that ASR on benign and adversary clients are highly correlated. Hence, for the adversary to ensure it can fool other clients in a black-box setting, it needs to obtain good results on its own data and model. So tuning the hyperparameters, data preprocessing can be all effective as long as they improve ASR on adversary.

\textbf{AETR/ASR difference:}, Attacks have higher AETR than ASR, which enables the adversary to subsample examples to achieve higher transferability. 
%. In black-box models, the attack results might vary from low transferability to similar to white-box. Depending on many parameters. But when implementing in a
% FL environment, the results are closer to the white-box setting. 
% This finding admits that models trained in FL setting keep their traditional ML vulnerabilities, and FL imposes an additional threat. Leading to aggregated vulnerabilty.\hl{  \faClockOshayad ye graph peyda Koni ke ASR ro ba white/black tozih bede}

\textbf{Attack domain}: We observed that transferability is specific within imaging domains, which is consistent with prior findings \cite{bortsova2021adversarial}. Attacks on Pathology images were consistently more successful than MRI images. 

% \subsection{Effect of parameters}
\textbf{Perturbation parameter}
% $\epsilon$  As shown in \ref{fig: epsilon graphs} 
Level of $\epsilon$ can substantially change transferability. Increasing $\epsilon$ does not improve ASR from a certain point, but adding CRN can increase the dependency. The best perturbation range in our experiments is around 0.03-0.05. These results suggest that conclusions in a centralized setting might not apply to a federated environment. And it shows different transferability behavior or parameter dependence.

\textbf{Step parameter } Our findings show that common $\alpha$ values have a  negligible effect on the final results, aside from too small or too large values. The reason could be that $\alpha$ similar to  $\epsilon$  bounds the change in each iteration, but generally, its values are one order of magnitude less than $\epsilon$. 


\subsection{Efficiency}
% Attacks can substantially differ in the computational requirements, 
% which can have practical implications in the MIA domain.
Our results show that computational complexity has a linear dependence on the number of iterations. However, the increase in transferability can vary. PGD with random intialization requires high computational power which might be burdensome for High-resolution or large-batch training. Also, if PGD performs poorly initially, having higher iterations does not help much.
Initialization can be influential in computational efficiency.  Using CRN leads to much fewer computational requirements. Single-step attacks can be $20 \sim 30 \times$ less expensive than iterative models with 40 iterations. Also, FGSM with CRN can outperform PGD with random initialization.\\
With less GPU requirements, adversaries might be capable of attacks using high-volumes of data or with multiple devices by using CRN.
\\
Standard ways of simulating attacks, like adaptive models and sanity checks, \cite{carlini2019evaluating} might be unfeasible in their traditional way. An adversary might have more knowledge than what is assumed in evaluation models, hence using more efficient methods or attacks with unexpected devices.



\subsection{Practical implications and suggestions}
Advanced fabrication algorithms and hard to detect methods are always intriguing for fraudsters. Existing Manipulations like altering the visual features of images, or using photo editing software, \cite{chowdhry2014image} can result in images of benign subjects classified as malignant,
\peter{This should be discussed in the introduction. The motivation and goal for the attacker seems unclear.}
\quickthings{I have moved some parts to the introduction and kepts some of it here. Hope it's okay now.}
 \peter{This seems to be a goal also of backdoor attacks which I think are more concerning than pure model poisoning. It would be interesting to see if the federated setting somehow affects the trained global model when the adversarial noise it added at test time. Are there any differences to models that are trained in a centralized fashion?}
\quickthings{Interesting point of view. Since it is in the test time, it is fundamentally different than backdoor, poisonining , flipping etc. which all happen during the training.. The question of those attacks are " how can we change the model parameters that for a set of non manipulated test data, we have a high classification error" 
 The question here is " How can we change the input test data, that for a set of not manipulated models, we have a high classification error", so maybe a better experiment would be with a radnom noise?}
 \cite{xia2020pseudo}\cite{sun2020adversarial}, but with visual distortion. In contrast, adversarial attacks are imperceptible, do not require manual intervention, and have high transferability. That gives a significant incentive for potential fraudsters to utilize adversarial attacks for high potential revenue. \\
% and send it to the target company.
% \\These vulnerabilities have some implications for clinical decision-makers, stakeholders, and insurance companies, who consider deploying federated or AI pipelines , which will be discussed in the following.
% \begin{enumerate}[(i)]
%     \item  First, manipulation and fraud is pervasive in healthcare and is reinforced by financial and personal incentives. This should be taken into consideration\cite{finlayson2019adversarial}.
%     \item Second, having a secure infrastructure in training phase does not guarantee safety in the deployment phase. So the difference between these two should be clear, and redundant ways might be considered to incorporate AI in medical image analysis pipelines.
% \item  Third, size and level of trust should be regarded as imporant parameters in collaborative/federated networks. Smaller networks with trusted parties have lower probability of having potential adversary.
% \item Fourth, Not enforcing same data pre-processing pipelines and using diverse data hinders the adversary. However, having disparate data comes with a compromise: it affects performance or even convergence of federated network \cite{li2019convergence}. So healthcare managers should consider whether it is worth sacrificing performance for security.
% \end{enumerate}
% \\Based on these findings, developers of medical image analysis systems should consider four things:
% \begin{enumerate}[(i)]
%     \item Developers can help end-users and clinicians by providing them more information other than model outputs. For example, adding explainable system reports helps the clinicians evaluate the legitimacy of predictions.
%     \item There are some suggestions by \cite{carlini2019evaluating} to test the adversarial robustness in centralized setting. Notably, performing adaptive attacks, with standard scenarios to disclose vulnerabilities. However, those ways are not recommended in a federated setting. Developers should consider scenarios where adversary traces the global model, and has more knowledge, or attacks with unexpected devices.
%     \item We saw that attack setting, and values of parameters like $\epsilon$, can affect transferability. Adversary might enhance its attack by choosing the right set of parameters and setting. However, there is no universal setting that guarantees a better performance. Hence,
%     % is no clear pr
%     % There are no universal factors, parameter or setting where the adversary to predict the capability of adversary, so 
%     developers are encouraged to use the results from prior  research to  find the optimal parameter set for their desired domain, or they should brute-force search to find upper-bounds of vulnerability \cite{carlini2019evaluating}. 
%      \item Despite not having a universal defense method, there are limited case-specific defense models shown to work on some datasets, \cite{graese2016assessing} so developers might consider looking into potential defense method for their usecase.
% \end{enumerate}
Such vulnerabilities entail implications for clinical decision-makers, stakeholders, and insurance companies considering the deployment of federated or AI pipelines, which we discuss below:

\begin{enumerate}[(i)]
\item Manipulation and fraud, pervasive in healthcare and reinforced by financial and personal incentives, must be considered\cite{finlayson2019adversarial}.
\item A secure infrastructure during training does not guarantee safety during deployment; therefore, the distinction must be clear, and alternative methods may be required to integrate AI into medical image analysis pipelines.
\item Size and trustworthiness are crucial parameters in collaborative/federated networks. Smaller networks with trusted parties reduce the likelihood of adversaries.
\item Employing diverse data and not enforcing uniform data pre-processing pipelines impedes adversaries. However, disparate data may compromise performance or convergence of federated networks \cite{li2019convergence}, necessitating healthcare managers to weigh security against performance.
\end{enumerate}

Developers of medical image analysis systems should consider the following:

\begin{enumerate}[(i)]
\item Providing end-users and clinicians with supplementary information, such as explainable system reports, to evaluate prediction legitimacy.
\item Employing suggestions from \cite{carlini2019evaluating} to test adversarial robustness in centralized settings is inadvisable in federated settings. Developers must consider scenarios where adversaries trace the global model and employ unexpected devices.
\item Attack settings and parameters like $\epsilon$ affect transferability. Adversaries may enhance attacks by selecting suitable settings. Developers should utilize prior research findings to determine optimal parameters for their domain or conduct brute-force searches to identify vulnerability upper bounds \cite{carlini2019evaluating}.
\item Although no universal defense method exists, limited case-specific defense models have proven effective on select datasets \cite{graese2016assessing}, warranting exploration of potential defense methods for specific use cases.
\end{enumerate}

\peter{Adding some discussion on how the attack could be detected would be good.}\quickthings{Added!}
Future lines of research could be to improve existing defense methods,\cite{li2022review,sun2019can,wang2020attack,shao2019stochastic} , towards a universal defense algorithm. Although there are some promising results, Some of them are only usable under specific settings\cite{yin2022adc},like they work for manipulations that cause a pattern that is previously known by the defender. Some of the algorithms require too much computational power  \cite{yuan2019adversarial,uesato2018adversarial,yin2022adc}, as they need to assume multiple scenarios and retrain the model on all of the corrupted samples generated from all those scenarios. Some detection models lead to drastic model parameter change\cite{zheng2020efficient}. Also, some recent studies have shown that the existing defense methods are ineffective if the adversary is aware of them \cite{yin2022adc}. 

Another line of research could be how to utilize distributed nature of federated networks to protect all participating clients, or if collaboration can be used to enhance the current defense methods.\\

% One implication it might give is that, we might increase the robustness of FL network, 


\section{Conclusion}
\label{sec:conclusion}

This paper investigated adversarial attacks on federated medical image analysis systems and discussed the crucial parameters on their transferability. It also proposed a new method that leverages the federated setting to improve the attack success rate and reduce the computation burden.
Our results indicate that tuning the parameters can substantially improve transferability.
It was also observed that adequately using noise from previous model updates can effectively improve computational load and has the potential to be well integrated into the existing attack methods.


We hope this research could benefit healthcare institutions and hospitals considering bringing in AI or joining fedrated networks to be more aware of the threat of adversarial examples. For medical institutions and managers of hospitals and insurance companies, this research suggests that they should pay extra attention to the AI pipelines and federated deployments. Our results indicate that security experts should re-asses standard vulnerability analysis and consider less common scenarios where a capable adversary proposes fast and efficient attacks. 
% For ML researchers involved in bringing in FL networks, a line of research can devise more reliable defense methods.

